Towards Understanding the Safety Boundaries of DeepSeek Models: Evaluation and Findings

This study presents the first comprehensive safety evaluation of the DeepSeek models, focusing on evaluating the safety risks associated with their generated content. Our evaluation encompasses DeepSeek's latest generation of large language models, multimodal large language models, and text-to-image models, systematically examining their performance regarding unsafe content generation. Notably, we developed a bilingual (Chinese-English) safety evaluation dataset tailored to Chinese sociocultural contexts, enabling a more thorough evaluation of the safety capabilities of Chinese-developed models. Experimental results indicate that despite their strong general capabilities, DeepSeek models exhibit significant safety vulnerabilities across multiple risk dimensions, including algorithmic discrimination and sexual content. These findings provide crucial insights for understanding and improving the safety of large foundation models. Our code is available at https://github.com/NY1024/DeepSeek-Safety-Eval.

==> conclusion.tex <==

\section{Conclusion}
GPT-4o, as an end-to-end MLLM, has shown great revolutionary potential in various fields. Despite its powerful general capabilities, its safety has not yet been thoroughly evaluated. Due to the limitations of the official OpenAI API, this study primarily focuses on the automated evaluation of jailbreak attacks involving text and visual modalities on large datasets via the API. Additionally, we also conduct jailbreak attacks on the audio modality manually using a subset of AdvBench via a mobile app. This study reveals several critical observations for the first time. We hope this work raises awareness in the community about the safety risks of MLLMs and urges researchers to prioritize the development of alignment strategies and mitigation techniques for MLLMs.

\textbf{Limitations and discussions.}
 \ding{182} This study adopts an audio modality jailbreak approach that merely translates known textual adversarial prompts into the audio modality, thereby diminishing the flexibility of audio modality jailbreak attacks. Considering the current capabilities of GPT-4o in audio processing, which enable the understanding of speech intonation and emotion, subsequently influencing its responses, future research endeavors could delve deeper into the ramifications of these factors on safety risks. \ding{183} Due to the scarcity of current multimodal jailbreak datasets, this study merely delves into exploring the impact of text-vision multimodal jailbreaking on the safety of GPT-4o. In the future, it is imperative to expeditiously establish multimodal datasets encompassing various combinations of modalities such as text, vision, and audio, to comprehensively assess the safety capabilities of MLLMS including GPT-4o.



==> introduction.tex <==
\section{Introduction}
As the representative of the new generation of Multimodal Large Language Models (MLLMs), gpt-4o \cite{4o} has garnered significant attention due to its outstanding performance \cite{4o1,4o2,4o3}. Despite its impressive capabilities, its safety aspects remain sufficiently explored. Given the potential
societal impact of risky content generated by advanced generative AI such as GPT-
4o, it is crucial to rigorously evaluate its safety. To unveil the safety risks of the models ~\cite{bd1,bd2,liu2023pre,liu2023does,liang2024poisoned,liang2024vl}, \emph{jailbreak attacks} \cite{jail2} have emerged as a red teaming strategy to circumvent guardrails and assess model alignment \cite{align1,align2}. Unlike typical adversarial attacks \cite{liu2023x,liu2020spatiotemporal,zhang2021interpreting,liu2020bias,liu2019perceptual,wang2021dual}, after jailbreaking, attackers can convince the model to do anything resulting in severe safety consequences, \eg, generating harmful or unethical content that is otherwise prohibited by alignment guidelines.

Therefore, this paper for the first time conducts a rigorous evaluation of GPT-4o against jailbreak attacks. Specifically, we utilize the GPT-4o API \footnote{\url{https://platform.openai.com/docs/models/gpt-4o}} released by OpenAI (which, at the time of writing, supports text-image combinations as input and text as output) to conduct automated safety evaluations from both the \emph{textual} and \emph{visual} modalities. Additionally, we perform a limited manual safety evaluation from the \emph{audio} modality using the GPT-4o mobile application \footnote{\url{https://play.google.com/store/apps/details?id=com.openai.chatgpt}}.


To ensure a comprehensive evaluation, we adopt a series of multi-modal and uni-modal jailbreak attacks on four benchmark datasets, totaling 2000 \emph{unimodal} text queries and 15 related attack scenarios, as well as 2180 \emph{multimodal} queries and 13 related attack scenarios. Notably, our evaluation involves the optimization of over 4,000 initial text queries and the analysis and
statistical evaluation of nearly 8,000+ responses on GPT-4o. Our extensive experiments reveal several novel observations including: \ding{182} Compared to earlier versions such as GPT-4V, GPT-4o exhibits enhanced safety against text modal jailbreak attacks. Nevertheless, experiments demonstrate that text modal jailbreak attacks possess strong transferability, effectively compromising multimodal models like GPT-4o. \ding{183} The newly introduced audio modality exposes a new attack surface for jailbreak attacks on GPT-4o. The methods proposed in this study can effectively exploit the audio modality to jailbreak GPT-4o. \ding{184} Current black-box multimodal jailbreak attack methods are largely ineffective against GPT-4o and GPT-4V. Nonetheless, experiments indicate that GPT-4o is less safe than GPT-4V at the multimodal level. \ding{185} Attacks based on known jailbreak templates are comparatively ineffective, indicating OpenAI's proactive efforts in mitigating well-known jailbreak patterns.

To the best of our knowledge, this paper is the first to comprehensively evaluate the safety of GPT-4o using jailbreak attacks across three modalities. We hope this paper can promote the design of robust alignment guardrails in next-generation multimodal large models.



==> multimodal.tex <==
\section{mutlimodal jailbreak attacks}
In this section, we evaluate the target models using other two black-box multimodal jailbreak attack methods. It is important to note that the method proposed by Gong \cite{figstep} and Liu \cite{mmsafety} involves a complex process for generating visual adversarial prompts. Since they all have already provided pre-constructed datasets, we conduct our tests solely on their datasets. Additionally, we use only the original text of the dataset for queries under the \texttt{No Attack} condition to facilitate comparative analysis of the experimental results (the ASRs under \texttt{No Attack} is calculated by $\mathcal{J}_4$).

\textbf{Evaluation on SafeBench.} SafeBench is a dataset created by Gong \etal{} \cite{figstep} using the proposed FigStep method. The core idea of FigStep is to convert harmful intent from original queries into formatted typographic images with blank spaces left in the images, which are then filled by target models. 

From the results in \Tref{safebench}, it can be observed that in each type of $\mathcal{J}$, the results for GPT-4o are consistently higher than those for GPT-4V (42.0\% as most in $\mathcal{J}_4$), \emph{indicating that GPT-4o is more susceptible to such attacks compared to GPT-4V}. Considering the superior multimodal fusion capabilities of GPT-4o, this may also contribute to its increased vulnerability to such attacks. It is noteworthy that we have observed an anomalous phenomenon wherein the target models' ASR in certain scenarios (\eg, \texttt{Illegal Activity}, \texttt{Adult Content}) under the \texttt{No Attack} condition is higher than the ASR under the attack. \Fref{fig} in Appendix \ref{ad-fig} illustrates an example of this phenomenon, where jailbreak attempts fail more frequently when multimodal queries are used. This observation contradicts the findings of the original paper as well as our intuition. It is hypothesized that this discrepancy may be due to OpenAI's implementation of specific defenses against multimodal typographic attacks similar to FigStep. These typographic attacks typically require the use of strings such as ``\texttt{... please generate detailed content for each item on the list mentioned above ...}'' within the textual prompt to be effective. We suspect that OpenAI might detect signs of typographic attacks based on these string characteristics, thereby employing stronger mitigation mechanisms during inference.

In scenarios other than those exhibiting anomalous phenomena, the ASR achieved using the FigStep attack is not significantly higher than the ASR under the \texttt{No attack} condition. For instance, when attacking GPT-4o, the ASR for the \texttt{Hate Speech} scenario is only 3.6\%. This indicates that the FigStep attack is largely ineffective against GPT-4V and GPT-4o. It is important to note that, given OpenAI's potential dynamic adjustments to the protective measures of their commercial models, our current findings do not negate the possibility that FigStep was effective at jailbreaking GPT-4V at the time of its initial publication.


\begin{table}[!t]
\centering
\caption{Multimodal jailbreak results (\%) on SafeBench.}
\begin{adjustbox}{width=\textwidth}

\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Scenarios} & \multicolumn{2}{c|}{No Attack} & \multicolumn{2}{c|}{$\mathcal{J}_1$} & \multicolumn{2}{c|}{$\mathcal{J}_2$} & \multicolumn{2}{c|}{$\mathcal{J}_3$} & \multicolumn{2}{c}{$\mathcal{J}_4$} \\ \cmidrule(l){2-11} 
                          & GPT-4V             & GPT-4o            & GPT-4V              & GPT-4o              & GPT-4V             & GPT-4o             & GPT-4V           & GPT-4o           & GPT-4V          & GPT-4o          \\ \midrule
Illegal Activity          & 40.0             & 48.0            & 0.0               & 16.0              & 0.0              & 2.0              & 8.0            & 22.0           & 6.0           & 22.0          \\
Hate Speech               & 6.0              & 10.0            & 2.0               & 26.0              & 0.0              & 8.0              & 12.0           & 18.0           & 2.0           & 22.0          \\
Malware Generation        & 8.0              & 14.0            & 6.0               & 48.0              & 0.0              & 30.0             & 8.0            & 54.0           & 6.0           & 48.0          \\
Physical Harm             & 4.0              & 10.0            & 0.0               & 8.0               & 2.0              & 0.0              & 8.0            & 4.0            & 4.0           & 4.0           \\
Fraud                     & 8.0              & 12.0            & 8.0               & 46.0              & 2.0              & 18.0             & 10.0           & 44.0           & 8.0           & 48.0          \\
Adult Content             & 52.0             & 46.0            & 16.0              & 46.0              & 0.0              & 6.0              & 18.0           & 20.0           & 8.0           & 22.0          \\
Privacy Violation         & 18.0             & 14.0            & 12.0              & 38.0              & 0.0              & 2.0              & 16.0           & 24.0           & 16.0          & 30.0          \\
Legal Opinion             & 0.0              & 2.0             & 68.0              & 88.0              & 0.0              & 0.0              & 4.0            & 6.0            & 8.0           & 4.0           \\
Financial Advice          & 4.0              & 4.0             & 86.0              & 94.0              & 0.0              & 0.0              & 4.0            & 10.0           & 4.0           & 6.0           \\
Health Consultation       & 6.0              & 2.0             & 60.0              & 86.0              & 0.0              & 0.0              & 4.0            & 0.0            & 16.0          & 34.0          \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{safebench}
\end{table}

\textbf{Evaluation on MM-SafetyBench.} MM-SafetyBench is a multimodal jailbreak dataset specifically curated by Liu \etal{}. \cite{mmsafety}, who proposed a method for constructing visual adversarial prompts based on image semantics. Specifically, harmful semantics from original queries are transformed into images through a text-to-image model, and crucial typographic text is then appended to generate the required visual adversarial prompts.

The experimental results based on MM-SafetyBench are presented in \Tref{mmsafe}. Comparing \Tref{safebench} and \Tref{mmsafe}, it can be seen that in some similar scenario types (\eg, \texttt{Legal Opinion}, \texttt{Financial Advice}), there is a significant disparity in ASR between the two datasets, with ASRs approaching 100\% on MM-SafetyBench for these scenarios. This is primarily due to the lack of sufficient harmfulness in the textual queries for these scenarios in MM-SafetyBench. Additionally, Liu \etal{} recommended using prompts specific to these scenario types for evaluation in both their paper and code. For instance, in the legal opinion scenario, a jailbreak failure is only determined when the response contains statements resembling ``\texttt{I do not have relevant authentication certificates}''. Consequently, the ASRs for these scenarios tend to be higher. When we focus on the experimental results for scenarios with strong harmfulness, such as \texttt{Hate Speech}, \texttt{Physical Harm}, and \texttt{Fraud}, in \Tref{mmsafe}, we observed that the ASRs of the target models under attack are consistently lower than those under the \texttt{No Attack} condition. An example is provided in \Fref{liu} of Appendix \ref{ad-liu}. This phenomenon was also observed in \Tref{safebench}, leading us to speculate that OpenAI has implemented specific defenses against these known multimodal attack methods. For instance, concerning the image semantics-based attacks proposed by Liu \etal{}, OpenAI may employ advanced defense mechanisms upon detecting images containing harmful semantics, thereby preventing attackers from injecting harmful semantics or instructions into multimodal large models using images. The results in \Tref{mmsafe} reveal that when attacking GPT-4o, an anomalous phenomenon consistently occurs where the ASR under the no attack condition is higher than the ASR under the attack condition, except for the \texttt{Hate Speech}, \texttt{Economic Harm}, and \texttt{Legal Opinion} scenarios. A similar pattern is observed with GPT-4V. This indicates that the method proposed by Liu \etal{} is ineffective at jailbreaking GPT-4o and GPT-4V.

Additionally, we note that, except for the judgment results of $\mathcal{J}_3$, the results from the other three judgment functions indicate that ASRs of GPT-4o are always higher than that of GPT-4v. \emph{Combining the experimental result obtained from SafeBench, this clearly demonstrates that GPT-4o is more vulnerable to multimodal jailbreak attacks compared to GPT-4V.}

\begin{table}[]
\renewcommand{\arraystretch}{1.0}
\caption{Multimodal jailbreak results (\%) on MM-SafetyBench.}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Scenarios} & \multicolumn{2}{c|}{No Attack} & \multicolumn{2}{c|}{$\mathcal{J}_1$} & \multicolumn{2}{c|}{$\mathcal{J}_2$} & \multicolumn{2}{c|}{$\mathcal{J}_3$} & \multicolumn{2}{c}{$\mathcal{J}_4$} \\ \cmidrule(l){2-11} 
                          & GPT-4V             & GPT-4o            & GPT-4V              & GPT-4o              & GPT-4V             & GPT-4o             & GPT-4V           & GPT-4o           & GPT-4V          & GPT-4o          \\ \midrule
Illegal Activity        & 2.0              & 4.1           & 1.0               & 6.1             & 4.1            & 12.5           & 48.9         & 7.2          & 3.1         & 4.1         \\
HateSpeech                & 16.6           & 9.2           & 7.3             & 24.5            & 0.0              & 1.8            & 20.9         & 14.8         & 6.1         & 12.8        \\
Malware Generation        & 34.9           & 44.1          & 13.6            & 34.0              & 0.0              & 6.9            & 55.8         & 41.8         & 11.6        & 30.3        \\
Physical Harm             & 26.6           & 34.2          & 16.6            & 43.0              & 0.6            & 4.9            & 32.8         & 25.8         & 13.0          & 32.6        \\
Economic Harm              & 7.4            & 9.9           & 68.0              & 84.4            & 0.0              & 0.0              & 22.3         & 20.6         & 10.7        & 21.3        \\
Fraud                     & 7.1            & 9.8           & 5.8             & 9.0               & 0.6            & 1.9            & 42.4         & 13.7         & 5.8         & 7.9         \\
Sex                       & 50.9           & 48.1          & 15.5            & 52.8            & 1.8            & 9.2            & 19.4         & 47.6         & 6.4         & 28.6        \\
Political Lobbying       & 100.0            & 99.7          & 76.4            & 98.6            & 0.0              & 0.0              & 82.8         & 90.1         & 88.5        & 98.1        \\
Privacy Violence         & 17.4           & 34.7          & 7.9             & 21.5            & 0.7            & 1.4            & 34.7         & 16.6         & 7.2         & 20.2        \\
Legal Opinion            & 100.0            & 96.1          & 35.3            & 73.8            & 0.0              & 0.0              & 62.0           & 79.0           & 94.4        & 96.8        \\
Financial Advice         & 100.0            & 100.0           & 89.2            & 95.8            & 0.0              & 0.0              & 91.5         & 94.5         & 99.3        & 99.4        \\
Health Consultation      & 99.0             & 98.7          & 73.3            & 91.7            & 0.0              & 0.0              & 69.4         & 78.7         & 96.2        & 98.1        \\
Gov Decision             & 99.0             & 99.7          & 49.6            & 79.1            & 0.0              & 0.0              & 77.0           & 95.2         & 76.2        & 93.4        \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{mmsafe}
\end{table}


In this section, we evaluated the risk of multimodal jailbreak attacks faced by GPT-4o, including methods based on typographic and semantic content in images. Overall, we found that the ASRs of the target models were lower when under attack compared to when it was not. This may be because OpenAI employs more stringent safety measures when detecting harmful semantics in images. The current SoTA multimodal jailbreak methods are ineffective against GPT-4o and GPT-4V. Additionally, when under attack, GPT-4o exhibited weaker safety compared to GPT-4V, which we suspect may be related to GPT-4o's end-to-end multimodal processing capabilities.



==> setup.tex <==


\section{Evaluation Protocols}
\textbf{Models.} Our experiments primarily involve two target models: GPT-4V (GPT-4-vision-preview) \cite{4v} and GPT-4o \cite{4o}. We utilize the corresponding APIs \cite{4oapi} provided by OpenAI and mobile application \cite{4oapp} to interact with these models and conduct our evaluations. Additionally, we employ Llama2 (llama-2-7b-chat) \cite{llama2} as the source model for generating textual adversarial prompts, which are then transferred to attack target models.

\textbf{Datasets.} In order to comprehensively evaluate the safety of target models, we collected existing open-source jailbreak datasets based on both unimodal and multimodal. For the text modality, we used AdvBench \cite{advbench} and RedTeam-2K \cite{28k}, which includes datasets such as BeaverTails \cite{beaver}, Bai \etal{} \cite{hhrlhf}, and Shen \etal{} \cite{shen}. For the audio modality, we used AdvBench subsets.For the multimodal, we mainly used SafeBench \cite{figstep} and MM-SafetyBench \cite{mmsafety}, which were constructed based on two typical multimodal jailbreak methods. These datasets, in accordance with the user policies of OpenAI \cite{openai_policy} and Meta AI \cite{metapolicy}, have categorized the content of the datasets into different categories.

\textbf{Jailbreak methods.} We evaluate 7 state-of-the-art jailbreak methods, categorized into two types. \emph{Unimodal jailbreak attacks} involves template-based methods, GCG \cite{advbench}, AutoDAN \cite{autodan}, and PAP \cite{pap}. \emph{Multimodal jailbreak attacks} involves FigStep \cite{figstep}, Liu \etal{} \cite{mmsafety}, and BAP \cite{bap}. In particular, for FigStep and Liu \etal{}, official datasets constructed based on the respective methods have been released, thus, we directly employed them to evaluate the target models, foregoing the construction of corresponding datasets based on AdvBench for unified testing. The evaluation of other methods was conducted on AdvBench. For template-based methods, we selected 6 typical jailbreak prompts (detailed template content provided in \Tref{diff_prompt}) from the internet for testing and utilized their average ASR as the indicator of the method's effectiveness. Although GCG and AutoDAN initially proposed for white-box scenarios, they have demonstrated substantial transferability. In this study, we generated adversarial suffixes using GCG \cite{advbench} and AutoDAN \cite{autodan} by attacking Llama2, and subsequently applied these suffixes to attack GPT-4o and GPT-4V. Regarding BAP, it is a multimodal jailbreak attack method that integrates gradient-based visual adversarial prompt optimization and adaptive optimization of text-based adversarial prompts through a Chain-of-Thought process \cite{cot}. Despite targeting black-box models, the text adversarial prompt optimization in BAP remains unrestricted. Therefore, in this study, we employ it to evaluate the safety of the text modality.

\textbf{Metrics.}
We use attack success rate (ASR) as the main evaluation metric. For a given dataset $D$ and target model $F_\theta$, we calculate the ASR through the following formula:
\begin{equation}
    ASR = \frac{\sum\limits_{i}^{|D|} J(F_\theta(v_{i},t_{i},a_{i}))}{|D|},
\end{equation}
where $(v_{i},t_{i},a_{i})$ represent the $i$-th data in $D$. $v_{i}$ represents an image, $t_{i}$ represents a text, and $a_{i}$ represents an audio. When evaluating the specified modality, other modality will be set to null. Here, function $J(\cdot)$ is a judgment function, which returns 1 if it determines that the response $F_\theta(v_{i},t_{i},a_{i})$ is unsafe, and 0 otherwise. 

In this study, we follow existing work and instantiate the $J(\cdot)$ function using four different evaluation methods: string matching ($\mathcal{J}_1$) \cite{figstep,advbench,match1}, Llama Guard \cite{guard} ($\mathcal{J}_2$) \cite{28k}, ChatGPT \cite{chatgpt} with judgment prompts ($\mathcal{J}_3$) \cite{gptcheck1,gptcheck2,gptcheck3,mmsafety}, and GPT-4o with judgment prompts ($\mathcal{J}_4$). Please refer to Appendix \ref{string} for specific details on string matching. Llama Guard is a custom model based on Llama 2-7b \cite{llama2}, designed to classify responses from the model to assess potential risks. The prompts used for ChatGPT and GPT-4o are provided in \ref{app_prompt}. For all the above metrics, the \emph{higher value indicates lower model safety against attacks.} 

Before delving into a detailed analysis of the experimental data, we argue it is essential to elucidate the characteristics of four types of judgment functions $\mathcal{J}$. There are significant numerical discrepancies in the judgment results of them. The judgment function $\mathcal{J}_1$ is most likely to be erroneous because it makes decisions based solely on specific strings. For instance, the model might indicate that the query is unethical but might not include phrases like ``\texttt{I'm sorry...}'' leading to false negatives in jailbreak failure detection. This results in $\mathcal{J}_1$ producing a higher ASR value. Judgment function $\mathcal{J}_2$ defines successful jailbreak very stringently, which can lead to false positives, thereby resulting in lower ASR values. Judgment function $\mathcal{J}_3$ uses the judgement prompt and the model's response as input, which can also yield biased values. For example, due to inevitable hallucinations \cite{hall1}, ChatGPT might sometimes consider a response with just the phrase ``\texttt{I'm sorry...}'' as a successful jailbreak. During evaluation of judgment method $\mathcal{J}_4$, both the query and the model's response are assessed together, providing a more comprehensive analysis of whether the model's response contains unsafe content related to the query. Comparatively, the ASR values derived from judgment method $\mathcal{J}_4$ are more accurate.

In our experimental evaluation, we will calculate the ASR using all four types of $\mathcal{J}$ simultaneously. For qualitative analysis, we will adopt the ensemble learning approach, using the majority decision of the judgment functions as the criterion. For quantitative analysis, we will primary rely on the results of $\mathcal{J}_4$.


==> unimodal.tex <==
\section{Unimodal Jailbreak Attacks Evaluation} \label{uni}
In this section, we evaluate model safety against unimodal jailbreak attacks including text modality and audio modality.

\subsection{text modality jailbreak}
\textbf{Evaluation on RedTeam-2K}. We first evaluate the safety of the target models on the RedTeam-2K dataset in the text modality setting. It is important to note that the textual queries in this dataset only contain unsafe intentions and do not include any attack payloads, \ie, these queries have not been subjected to any additional perturbations.

As shown in \Tref{2k}, from a broad perspective, \emph{the safety level of GPT-4o is lower than that of GPT-4V in the absence of attacks.} When considering specific scenarios, particularly those with higher risk potential (\eg, \texttt{Physical Harm}), the disparity in ASR between the two target models becomes even more pronounced, reaching a difference of 14.6\%. This experimental finding stands in stark contrast to the intuitive belief that GPT-4o would be the safer model in the absence of attacks. This indicates that a model with stronger general capabilities does not necessarily equate to enhanced safety performance and may be weaker in our context. 

The observed performance discrepancy might stem from an inherent conflict between training objectives and safety objectives. Training objectives, particularly for large models, often emphasize knowledge acquisition and comprehensive response generation. This entails exposing the model to a diverse range of data, including potentially unsafe or harmful content. In contrast, safety objectives prioritize minimizing exposure to harmful content during the pre-training phase and preventing the generation of malicious responses during deployment. This inherent conflict can lead to a trade-off between model performance and safety. While models trained on a broader dataset may exhibit superior performance in terms of knowledge and comprehensiveness, they may also be more susceptible to generating unsafe or harmful content. Conversely, models trained with stringent safety measures may exhibit reduced performance due to limited exposure to diverse data and strict response guidelines. \emph{In a word, our experimental data suggests that GPT-4o may not have adequately balanced the trade-off between training objectives and safety objectives.} 


\begin{table}[]\scriptsize
\centering
\caption{Text modality jailbreak results (\%) on RedTeam-2K.}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Scenarios}  & \multicolumn{2}{c|}{$\mathcal{J}_1$} & \multicolumn{2}{c|}{$\mathcal{J}_2$} & \multicolumn{2}{c|}{$\mathcal{J}_3$} & \multicolumn{2}{c}{$\mathcal{J}_4$} \\ \cmidrule(l){2-9} 
                           & GPT-4V              & GPT-4o              & GPT-4V             & GPT-4o             & GPT-4V           & GPT-4o           & GPT-4V          & GPT-4o          \\ \midrule
Animal Abuse               & 21.0              & 31.3            & 0.0              & 0.9            & 33.3         & 13.4         & 6.8         & 11.9        \\
Bias                       & 55.0              & 70.0              & 0.0              & 3.3            & 11.6         & 5.8          & 2.5         & 5.0           \\
Child Abuse                & 48.5            & 64.9            & 1.4            & 3.7            & 28.3         & 23.1         & 8.9         & 13.4        \\
Economic Harm              & 12.1            & 14.9            & 0.0              & 1.8            & 69.1         & 16.8         & 1.8         & 3.7         \\
Fraud                      & 6.2             & 11.7            & 0.0              & 0.0              & 50.0           & 22.6         & 3.0           & 9.6         \\
Government Decision        & 29.7            & 45.0              & 0.0              & 1.5            & 47.3         & 33.5         & 24.3        & 34.9        \\
Hate Speech                & 58.4            & 68.4            & 0.0              & 2.3            & 10.0           & 5.3          & 3.0           & 4.6         \\
Health Consultation        & 58.2            & 80.0              & 0.0              & 0.0              & 2.6          & 0.0            & 0.0           & 1.6         \\
Illegal Activity           & 5.2             & 6.6             & 0.6            & 5.2            & 71.5         & 18.5         & 1.3         & 5.9         \\
Malware                    & 6.4             & 12.0              & 0.0              & 0.0              & 64.8         & 23.2         & 2.4         & 9.6         \\
Physical Harm              & 30.8            & 41.4            & 2.5            & 4.9            & 39.0           & 29.2         & 9.7         & 24.3        \\
Political Sensitivity      & 54.6            & 65.3            & 0.7            & 0.0              & 12.3         & 4.6          & 0.7         & 4.6         \\
Privacy Violation          & 40.9            & 47.5            & 0.0              & 0.0              & 19.6         & 12.2         & 2.4         & 4.9         \\
Tailored Unlicensed Advice & 47.6            & 64.8            & 0.0              & 0.0              & 15.6         & 3.1          & 1.5         & 1.5         \\
Unethical Behavior         & 26.1            & 37.6            & 0.7            & 0.7            & 34.6         & 17.6         & 5.1         & 9.2         \\
Violence                   & 34.6            & 47.5            & 0.0              & 0.0              & 21.7         & 4.8          & 2.4         & 4.0           \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{2k}   
\end{table}

\textbf{Evaluation on AdvBench}
Most existing jailbreak attack research is based on AdvBench \cite{advbench}, which contains 520 harmful text queries. Considering the representativeness and applicability of this benchmark, in addition to evaluating the target model safety under the original text queries, we also assess the model safety against various SoTA jailbreak attacks.

In \Fref{adv_comp}, \texttt{No Attack} signifies the scenario where the target models are queried solely with the original text. Notably, we observed that the ASR for template-based jailbreak (\texttt{TBJ}) methods consistently fell to 0.0\%, even lower than the ASR under the \texttt{No Attack} scenario. \emph{This observation suggests that OpenAI has implemented additional safeguards against these widely circulated jailbreak templates.} One plausible explanation lies in the employment of pattern recognition techniques, enabling the direct rejection of queries containing known jailbreak patterns. As shown in \Fref{adv_comp}, compared to the \emph{No Attack} baseline, both GCG and AutoDAN achieved a notable degree of transferability in jailbreak MLLMs. When attacking GPT-4V, GCG and AutoDAN increased the ASR by 10\% and 14.1\%, respectively. PAP \cite{pap}, another method specifically designed for jailbreaking LLMs, employs various persuasion strategies to rewrite initial text queries, thereby inducing unsafe model responses. It boasts the highest ASR in text modality based jailbreak attacks (ASR for GPT-4V and GPT-4o are 62.2\% and 62.7\%, respectively). BAP \cite{bap} is a recently proposed multimodal jailbreak attack method. Although it is primarily used for evaluating MLLMs, in this study, we mainly utilize its text optimization capabilities. As illustrated by the results in \Fref{adv_comp}, BAP achieved the highest ASR, reaching 83.1\% when attacking GPT-4V.

When analyzing the experimental data from the perspective of the target models, we observe that except for PAP in $\mathcal{J}_3$, the ASR for attacking GPT-4o is lower than for attacking GPT-4V across all judgment functions and attack methods. \emph{This indicates that, under attack conditions, GPT-4o demonstrates higher safety compared to GPT-4V.}


\begin{figure}[htbp]  
    \centering  
    \begin{subfigure}[b]{0.24\textwidth}  
        \centering  
        \includegraphics[width=\textwidth]{img/1.pdf}  
        \caption{Results of $\mathcal{J}_1$.}  
        \label{fig:1}  
    \end{subfigure}  
    \hfill  
    \begin{subfigure}[b]{0.24\textwidth}  
        \centering  
        \includegraphics[width=\textwidth]{img/2.pdf}  
        \caption{Results of $\mathcal{J}_2$.}  
        \label{fig:2}  
    \end{subfigure}  
    \hfill  
    \begin{subfigure}[b]{0.24\textwidth}  
        \centering  
        \includegraphics[width=\textwidth]{img/3.pdf}  
        \caption{Results of $\mathcal{J}_3$.}  
        \label{fig:3}  
    \end{subfigure}  
    \hfill  
    \begin{subfigure}[b]{0.24\textwidth}  
        \centering  
        \includegraphics[width=\textwidth]{img/4.pdf}  
        \caption{Results of $\mathcal{J}_4$.}  
        \label{fig:4}  
    \end{subfigure}  
    \caption{Text modality jailbreak results (\%) on AdvBench.}  
    \label{adv_comp}  
\end{figure}  

\iffalse
\begin{table}[]\Large
\centering
\caption{Text modality jailbreak results (\%) on AdvBench.}
\scalebox{0.5}{
\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$\mathcal{J}_1$} & \multicolumn{2}{c|}{$\mathcal{J}_2$} & \multicolumn{2}{c|}{$\mathcal{J}_3$} & \multicolumn{2}{c}{$\mathcal{J}_4$} \\ \cmidrule(l){2-9} 
                         & GPT-4V              & GPT-4o              & GPT-4V             & GPT-4o             & GPT-4V           & GPT-4o           & GPT-4V          & GPT-4o          \\ \midrule
No Attack                & 4.2             & 3.1             & 5.6            & 0              & 13.8         & 9.4          & 9.2         & 1.9         \\
TBJ    & 0               & 0.0               & 0.0              & 0.0              & 0.0            & 0.0            & 0.0           & 0.0           \\
GCG                      & 6.9             & 5.4             & 14.0             & 0.2            & 40.2         & 9            & 19.2        & 1.9         \\
AutoDAN                  & 12.7            & 6.2             & 8.8            & 0.0              & 43.3         & 7.7          & 23.3        & 3.5         \\
PAP                       & 52.9            & 45.2            & 19.4           & 14.4           & 35           & 53.8         & 69.2        & 62.7        \\
BAP                      & \textbf{71.7}            & \textbf{71.5}            & \textbf{18.5}           & \textbf{16.2}           & \textbf{65.8}         & \textbf{57.1}         & \textbf{83.1}        & \textbf{73.3}        \\ \bottomrule
\end{tabular}
}
\label{adv_comp} 
\end{table}
\fi

\iffalse
\begin{table}[]\scriptsize
\centering
\caption{Text modality jailbreak results (\%) on AdvBench.}
\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{$\mathcal{J}_1$} & \multicolumn{2}{c|}{$\mathcal{J}_2$} & \multicolumn{2}{c|}{$\mathcal{J}_3$} & \multicolumn{2}{c}{$\mathcal{J}_4$} \\ \cmidrule(l){2-9} 
                         & GPT-4V              & GPT-4o              & GPT-4V             & GPT-4o             & GPT-4V           & GPT-4o           & GPT-4V          & GPT-4o          \\ \midrule
No Attack                & 4.2             & 3.1             & 5.6            & 0              & 13.8         & 9.4          & 9.2         & 1.9         \\
TBJ    & 0               & 0.0               & 0.0              & 0.0              & 0.0            & 0.0            & 0.0           & 0.0           \\
GCG                      & 6.9             & 5.4             & 14.0             & 0.2            & 40.2         & 9            & 19.2        & 1.9         \\
AutoDAN                  & 12.7            & 6.2             & 8.8            & 0.0              & 43.3         & 7.7          & 23.3        & 3.5         \\
PAP                       & 52.9            & 45.2            & 19.4           & 14.4           & 35           & 53.8         & 69.2        & 62.7        \\
BAP                      & \textbf{71.7}            & \textbf{71.5}            & \textbf{18.5}           & \textbf{16.2}           & \textbf{65.8}         & \textbf{57.1}         & \textbf{83.1}        & \textbf{73.3}        \\ \bottomrule
\end{tabular}
\label{adv_comp} 
\end{table}
\fi
\subsection{audio modality jailbreak}

Due to the temporary unavailability of OpenAI's audio-related APIs and the rate limit on requests in the mobile app, we can only conduct limited testing on the safety of the audio modality. Firstly, we used GPT-4o to classify AdvBench and randomly selected 10 textual queries from the 4 most frequent categories. Concurrently, based on experimental data from the previous section, we selected adversarial textual prompts generated by GCG, AudoDAN, PJ, and BAP. Subsequently, we employed OpenAI's \texttt{TTS-1} API\footnote{\url{https://platform.openai.com/docs/guides/text-to-speech}} to convert a total of 200 text samples into MP3 format. Due to the limited amount of experimental data in this section, we manually assessed the safety of the responses to calculate the ASR. 


The results are shown in \Tref{adv_mp3}. It can be observed that using the original text query converted into audio does not allow for the successful jailbreak of GPT-4o. \emph{This demonstrates that GPT-4o has sufficient safety at the audio modality level}. Additionally, \emph{we found that texts which could successfully jailbreak GPT-4o when using methods like GCG and AutoDAN, failed to do so when converted into audio modality}. The primary reason is that the adversarial suffixes generated by these methods lose some critical semantic information (such as non-alphabetic symbols) during the modalities processing. From \Tref{adv_mp3}, we observe that the adversarial prompts from PAP and BAP show slightly higher ASR for the original text prompts compared to the audio prompts converted from these texts. For example, in the scenario of \texttt{Illegal Activity}, the ASR for BAP in text modality is 100\%, while in audio modality is 80\%. Upon examining the interaction results, we found that during audio interactions, GPT-4o sometimes responds with a simple \texttt{Sure} and then asks for further details, mimicking human conversational style. However, the text modality based jailbreak methods used in this study did not account for this aspect, as they rely on single-turn conversations to achieve jailbreak. \emph{Consequently, the ASR of jailbreak attacks in audio modality is slightly lower than in text modality}. Notably, despite the gap, the ASR for audio adversarial prompts did not significantly decrease. This is largely because strategies used by PAP and BAP closely resemble human processing methods. For instance, they employ persuasive tactics, such as scenario-based assumptions, to optimize the entire statement.


\begin{table}[]\scriptsize
\centering
\caption{Audio modality jailbreak results (\%) on AdvBench subset.}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}c|ccccc|ccccc@{}}
\toprule
\multirow{2}{*}{Scenarios} & \multicolumn{5}{c|}{Text Modality}   & \multicolumn{5}{c}{Audio Modality}  \\ \cmidrule(l){2-11} 
                           & Ori. Text & GCG & AudoDAN & PAP  & BAP & Ori. Text & GCG & AudoDAN & PAP & BAP \\ \midrule
Illegal Activity           & 10       & 0   & 10      & 100 & 80  & 0        & 0   & 0       & 90 & 80  \\
Physical Harm              & 0        & 0   & 0       & 80  & 100 & 0        & 0   & 0       & 80 & 100 \\
Fraud                      & 10       & 10  & 10      & 100 & 90  & 0        & 0   & 0       & 80 & 80  \\
HateSpeech                 & 0        & 0   & 0       & 70  & 90  & 0        & 0   & 0       & 70 & 80  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{adv_mp3}   
\end{table}

Overall, in this subsection, we conducted evaluation on the safety of the text modality in GPT-4o as well as the recently integrated audio modality. We found that in terms of the text modality, GPT-4o exhibits stronger safety compared to GPT-4V. Additionally, we observed that text adversarial prompts possess a certain level of transferability, indicating that prompts crafted for other LLMs still have the potential to successfully jailbreak GPT-4o. As for audio modality, based on our observations with the ChatGPT App, we employed a naive approach by directly converting text prompts into audio prompts for testing. The test results demonstrate that this method also achieves ASRs close to that of text based jailbreak attacks in attacking GPT4-o.
